On Decidability Timed Automata with 2 Parametric Clocks

In this paper, we introduce a restriction of Timed Automata (TA), called non-resetting test Timed Automata (nrtTA). An nrtTA does not allow to test and reset the same clock on the same transition. The model has the same expressive power of TA, but it may require one more clock than an TA to recognize the same language. We consider the parametric version of nrtTA, where one parameter can appear in clock guards of transitions. The focus of this draft is to prove that the $\omega$-language emptiness problem for 2-clock parametric nrtTA is decidable. This result can be compared with the parametric version of TA, where the emptiness problem for 2-clock TA with one parameter is not known to be decidable. Our result, however, extends the known decidability of the case of TA with one clock and one parameter from finite words to infinite words.

==> OverCmax.tex <==
\begin{itemize}

\item 
Let us consider an \rtor$_{\intprm}$ symbolic sequence $\rho = \region{R_0} \region{R_1} \ldots \region{R_{n-1}} \region{R_{n}}$ such that $\set{x = 0} \subseteq \region{R_0}$ holds.
For each $1 \leq j \leq n$, we associate with $\rho$ the \emph{induced constraints} %
defined in figures \ref{fig:overCmaxRj1}-\ref{fig:overCmaxR0} (where $0 < \const, \const' \leq \cmax$, $0 \leq \const''  < \cmax$), depending on the constraints that appear in $\region{R_0}$ and $\region{R_j}$.
\todoMR{}{Tabelle dovrebbero tutte sparire}
\todoMR{}{Occorre spiegare bene che i vincoli della figura \ref{fig:overCmaxRn} in realtà riguardano quello che viene dopo $\rho$ e non $\rho$ stessa.}



\begin{figure}[!ht]
{\color{red}
$\begin{array}{|c|c|c|c|}
\hline
                      & \multicolumn{3}{c} {\region{R_j} \text{ with } \set{y < \param} \subseteq \region{R_j}}\\\hline
      \region{R_0}    & \const’-1 < x < \const’         &  x = \const'                   &  x > \cmax                   \\\hline
\const-1 < y < \const & \intprm \geq \const + \const’ -2            &  \intprm \geq \const + \const’ -1        &  \intprm \geq \const + \cmax -1 \\\hline
y = \const            & \intprm \geq \const + \const’ -1            &  \intprm \geq \const + \const’           &  \intprm \geq \const + \cmax \\\hline
y \geq \cmax + \const''  & \intprm \geq \min \set{\cmax + \const’ + \const''-1, 2\cmax}  &  \intprm \geq \min \set{\cmax + \const’ + \const'', 2\cmax} &  \intprm \geq 2\cmax \\\hline
\end{array}$
\caption{Induced constraints to be associated with $\rho$ if there is a region $\region{R_j}$ in which constraint $y < \param$ appears.}
\label{fig:overCmaxRj1}
}
\end{figure}



\begin{figure}[!ht]
\color{red}
$\begin{array}{|c|c|c|c|}
\hline
                      & \multicolumn{3}{c} {\region{R_j} \text{ with } \set{y = \param} \subseteq \region{R_j}}\\\hline
      \region{R_0}    & \const’-1 < x < \const’                                       &  x = \const'                                                &  x > \cmax                   \\\hline
\const-1 < y < \const & \intprm \in \set{\const + \const’ -2, \const + \const’ -1}    &  \intprm = \const + \const’ -1                              &  \intprm \geq \const + \cmax -1 \\\hline
y = \const            & \intprm = \const + \const’ -1                                 &  \intprm = \const + \const’                                 &  \intprm \geq \const + \cmax \\\hline
y > \cmax +\const''   & \intprm \geq \min \set{\cmax + \const’ + \const''-1, 2\cmax}  &  \intprm \geq \min \set{\cmax + \const’ + \const'', 2\cmax} &  \intprm \geq 2\cmax \\\hline
y = \cmax +\const''   & \intprm = \min \set{\cmax + \const’ + \const''-1, 2\cmax}  &  \intprm = \min \set{\cmax + \const’ + \const'', 2\cmax} &  \intprm \geq 2\cmax \\\hline
\end{array}$
\caption{Induced constraints to be associated with $\rho$ if there is a region $\region{R_j}$ in which constraint $y = \param$ appears.}
\label{fig:overCmaxRj2}
\end{figure}


\begin{figure}[!ht]
\color{red}
$\begin{array}{|c|c|c|c|}
\hline
                      & \multicolumn{3}{c} {\region{R_j} \text{ with } \set{\param < y} \subseteq \region{R_j}}\\\hline
      \region{R_0}    & \const’-1 < x < \const’         &  x = \const'                   &  x > \cmax                   \\\hline
\const-1 < y < \const & \intprm < \const + \const’ &  \intprm < \const + \const’ &  \top \\\hline
y = \const            & \intprm < \const + \const’   &  \intprm < \const + \const’ &  \top \\\hline
y > \cmax             & \top     &  \top &  \top \\\hline
\end{array}$
\caption{Induced constraints to be associated with $\rho$ if there is a region $\region{R_j}$ in which constraint $\param < y$ appears.}
\label{fig:overCmaxRj3}
\end{figure}










\begin{figure}[!ht]
\color{red}
$\begin{array}{|c||c|c||c|c}
\hline
\multirow{2}{*}{$\region{R_0}$}  & \multicolumn{2}{c|} {\region{R_j} \text{ with } \set{y < \param, y = \param} \cap \region{R_j} \neq \emptyset} & \multicolumn{2}{c|} {\region{R_n} \text{ with } \set{y < \intprm -\const} \cap \region{R_n} \neq \emptyset}\\
                      & \const’-1 < x < \const’   &  x = \const'                &  \const’-1 < x < \const’   &  x = \const'               \\\hline\hline
y > \cmax             & y < \intprm - \const' + 2 &  y < \intprm - \const' +1   &   y < \intprm - \const - \const' + 1 &  y < \intprm - \const - \const' \\\hline
\end{array}$
\caption{Constraints to be associated with $\region{R_0}$ depending on the constraints that appear in some $\region{R_j}$, with $1 \leq j \leq n$.}
\label{fig:overCmaxR0}
\end{figure}


\end{itemize}




==> nrtTAproperties.tex <==

Consider the family of timed languages $\{L_k\}_{k > 0}$ where $L_k$ is the set of timed words over the alphabet $\{a\}$ such that there are at least $k$ distinct pairs of $a$'s at exactly distance $1$.
In \cite{PS12} it was shown that every $L_k$ is accepted by a TA with $k$ clocks, but it cannot be accepted by any TA with $k-1$ clocks. 
Formally, $L_k$ is the set of timed words of the form $(\pi,\tau)$, where $\pi:\Nat\to\{\emptyset, \{a\}\}$, $\pi(i) = \{a\}$ for every $i>0$
and there exist at least $k$ distinct pairs  $(i,j)$, $0<i<j\in \Nat$, such that $\tau(j)-\tau(i) = 1$.
\todoMR{}{in realtà dovrebbe essere $\pi(i) = a$, senza il set, no? Anche la signature di $\pi$ va rivista}




\begin{figure}[!tp]
    \centering
    \includegraphics[scale=0.5]{figs/nrtTA-L2.pdf}
    \caption{NrtTA with 2 clocks recognizing timed language $L_2$.}
    \label{fig:nrtTA-L2}
\end{figure}

It is easy to see that the nrtTA of Figure \ref{fig:nrtTA-L2}, which uses two clocks $x_1$ and $x_2$, recognizes language $L_2$.
Also, for any $k > 1$, a similar nrtTA with $k$ clocks that recognizes $L_k$ can be defined.


The  result can be generalized to 1-parametric TA, by considering the family of timed languages $\{L^{p}_{k} \mid {k > 0}\}$ where $L^{p}_k$ is the set of timed words 
over the alphabet $\{a\}$ such that there exist a real value $0< \delta\le 1$ and at least $k$ distinct pairs of $a$'s 
at exactly distance $\delta$. Formally, each language $L^p_{k}$ is the set of timed words of the form $(\pi,\tau)$, where $\pi:\Nat\to\{\emptyset, \{a\}\}$, $\pi(i) = \{a\}$ for every $i>0$ and there exist $0<\delta\le 1$ and at least $k$ distinct pairs  $(i,j)$, $0<i<j\in \Nat$, such that $\tau(j)-\tau(i) = \delta$. 

It is fairly obvious to define a 1-parametric TA with $k$ clocks recognizing $L^p_{k}$ and also to generalize the construction of Figure~\ref{fig:nrtTA-L2} to a 1-parametric nrtTA (just replace the constant 1 in the guards with the parameter). Therefore, $L^p_{k}$ can be recognized by a 1-parametric nrtTA with $k$ clocks. We now show that there is no 1-parametric TA (hence, not even a 1-parametric nrtTA) with $k-1$ clocks recognizing $L^p_{k}$. 



\begin{lemma}
    \label{lm:LPk-not-k-1}
    There exists a family of timed languages $\{L(k,n)\mid n, k \geq 1\}$
    such that each $ L(k,n)$ can be recognized by a parametric nrtTA with $k$ clocks and $n$ parameters, but 
    \begin{enumerate} \item $ L(k,n)$ cannot be recognized by a parametric TA with $k-1$ clocks and $n$ parameters; 
        \item $L(k,n)$ cannot be recognized by a parametric TA with less than $n$ parameters (regardless of the number of clocks).
    \end{enumerate}
\end{lemma}
\begin{proof}
    Let $k\ge 2$ (the case $k=1$ is obvious, since a TA with $k-1=0$ clocks is a finite-state automaton). %
    
    
    
    Consider the language $\bar{L}^{p}_k$, defined as the concatenation of the language ${L}_k$ with $(L^{p}_k)^n$, where $(L^p_{k})^n$ is the language obtained by $n-1$ concatenations of $L^p_{k}$ with itself.
    It is easy to see that $\bar{L}^{p}_k$ can be recognized by a parametric nrtTA with $k$ clocks and $n$ parameters.
    
    Assume by contradiction that there is a parametric TA $\A$ recognizing $\bar{L}^{p}_k$ with $n$ parameters and less than $k$ clocks, or with less than $n$ parameters (and an arbitrary number of clocks). 
    Let $\cmax\ge 1$ be the largest constant in the guards of $\A$.
    Consider first the case of $k-1$ clocks and $n$ parameters. We follow a similar argument to the one in \cite{PS12}, but applied to  $\bar{L}^{p}_k$.
    
    
    
    
    Consider a finite timed word  $(\pi,\tau)$ in $\bar{L}^{p}_k$,  with $2k(n+1)$
    instants, such that the first $k$ positions are included in the interval $(0,1)$, the next $k$ positions, between $k+1$ and $2k$, are included in $(1,2)$, and the remainder of the timed word, composed of exactly $n$ sets of $k$ pairs,  has timestamps greater than $\cmax$. 
    
    We can thus partition $(\pi,\tau)$ into $n+1$ sets $S_0, S_1, \dots, S_n$ of consecutive $2k$ positions, i.e., 
    $S_j = \{2kj+i\mid 1\le i \le 2k \}$, with $0\le j \le n$. 
    
    Each position of the form $(2kj+i)$ in a set $S_j$, $1\le i \le k, 0\le j \le n$ is called a {\em parent}, while position $(2kj+k+i)$ is called its {\em child}. 
    
    By the argument of \cite{PS12}, if no comparison with parameters is used in the run of the TA over the prefix in $L_k$, then the word cannot be accepted by a TA with less than $k$ clocks. 
    Hence, we assume that we may use less than $k$ clocks and one or more of the parameters, which must be matched for equality during the the run over the prefix. 
    
    
    
    
    
    Let $\delta_0=n+\cmax$ and for all $1\leq j\le n$, let $\delta_j=2*\delta_{j-1} = 2^{j}\delta_0$. 
    Also,  let 
    $$d_0=0 \text{ and for all } 1\leq j\le n \; \text{ it holds that } d_j = 1+\delta_{j-1} + d_{j-1}.$$
    
    Hence, $d_j= j+\sum_{i=0}^{j-1}\delta_i= j+ \delta_0+2\delta_0 + \dots 2^{j-1}\delta_0= j+(2^{j}-1)\delta_0$.  
    We now define the timestamps of $(\pi,\tau)$. 
    
    \begin{itemize}
        \item The timestamp of the leftmost parent $h=2kj+1$ of set $S_j$, $0\le j\le n$  is
        $\tau(h)= d_{j}-\frac{j+1}{2^n}$
        and for every $h<m< h+k$, 
        $\tau(m)= \tau(m-1)+ \frac{1}{2^{n+m}};$
        \item each parent-child pair in set $S_j$ is at distance $\delta_j$.
    \end{itemize}  
    
    For instance, to illustrate the above formula, the timestamps of the parents in set $S_0$ are included in the interval, 
    $\left[1-\frac{1}{2^n}, 1\right),$
    those in  set $S_1$ are  in the interval 
    $\left[\delta_0+1-\frac{2}{2^n}, \delta_0+1\right)$, those in  set $S_2$ are  in the interval 
    $\left[\delta_0+\delta_1 + 2-\frac{3}{2^n}, \delta_0+\delta_1+2\right),$ etc.---that is, each interval is smaller than $1$.
    
    
    We claim that for all arbitrary positions  $m,h$ of $(\pi,\tau)$ with $1\le h<m \leq 2k(n+1)$,
    such that $m$ is not the child of $h$,
    and for all positions  $m',h'$, with $h\le h'<m' \leq 2k(n+1)$,
    the timed word $(\pi,\tau)$ is such that
    
    \begin{equation}\label{eq-allDistinct}
        \text{if } \tau(m)-\tau(h)= \tau(m')-\tau(h') 	\text{ then } m=m' \land h=h'.
    \end{equation}
    
    
    We first prove Claim~\eqref{eq-allDistinct}
    \todoMR{}{e se ne dessimo anche una descrizione a parole?}
    for all parents  $h,m,h',m'$ of $(\pi,\tau)$.
    
    Hence, the timestamps of $\tau$ are such that the distance in time between any two parents is different 
    from any other distance between any other pair of parents. %
    
    Claim~\eqref{eq-allDistinct} can easily be verified  when each pair of parents is in the same set, that is, a pair of parents $h, h+q$ is in set $S_j$, and another pair of parents $h', h'+q'$ is in $S_{j'}$, with $j' \geq j$.
    In fact, the time distance $\tau(h+q)-\tau(h)$ between two parents $h,h+q$, with $0<q< k$, both in $S_j$, when $k\ge 2$ is:
    
    $$\tau(h+q)-\tau(h)= 
    \sum_{i=h+1}^{h+q}\frac{1}{2^{n+i}} = 
    \frac{1}{2^{n+h}} \sum_{i=1}^{i=q}\frac{1}{2^i} = \frac{1}{2^{n+h}} (1-\frac{1}{2^q})<1.$$
    
    The distance between one parent in position $h'>h$ and another parent, in position $h'+q'$, with  both positions in the same set $S_{j'}$ (with $0<q'< k$), is thus 
    $\tau(h'+q')-\tau(h')=\frac{1}{2^{n+h'}} (1-\frac{1}{2^{q'}})$. 
    \begin{align*}
        \tau(h+q)-\tau(h)=&\frac{1}{2^{n+h}} (1-\frac{1}{2^q})\ge\frac{1}{2^{n+h}}\frac{1}{2}= \frac{1}{2^{n+h+1}}>
        \\ &  \frac{1}{2^{n+h+1}} (1-\frac{1}{2^{q'}}) \ge \frac{1}{2^{n+h'}} (1-\frac{1}{2^{q'}})= \tau(h'+q')-\tau(h').	
    \end{align*}
    
    
    
    
    Consider now the case when comparing two parents $m,h$ in different sets $S_j,S_{j'}$ with $j'>j$.
    
    If $m$ is the leftmost parent of set $j'$ and $h$ is the leftmost parent of set $j$ then:
    
    \begin{equation}\label{eq-distanceLeftRight}
        \tau(m)-\tau(h)= d_{j'}-\frac{j'+1}{2^n} -d_{j}+\frac{j+1}{2^n} = j'-j+ \delta_{j'-1} + \delta_{j'-2} + \dots +\delta_{j} - \frac{j'-j}{2^n}.\
    \end{equation}
    The integer part of $\tau(m)-\tau(h)$ is thus 
    
    \begin{equation}\label{eq-Delta-ij}
        \Delta_{j',j} = j'-j-1 + \delta_{j'-1} + \delta_{j'-2} + \dots +\delta_{j}.
    \end{equation}
    Suppose now that there are $r'>r$, with $r'\neq j'$, such that the first parent, say $m'$, in set $S_{r'}$ and the first parent, say, $h'$  of set $S_{r}$ have a distance whose integer part is  equal to $\Delta_{j',j}$.
    As above,
    
    \begin{equation*}
        \tau(m')-\tau(h')= r'-r+ \delta_{r'-1} + \delta_{r'-2} + \dots +\delta_{r} - \frac{r'-r}{2^n}.
    \end{equation*}
    Hence, the integer part  of this distance is $\Delta_{r',r} = r'-r-1 + \delta_{r'-1} + \delta_{r'-2} + \dots +\delta_{r}$.
    To have the same distance, it must be that $r'-r=j'-j$ (since $j'-j<n<\delta_1$).
    
    Therefore, if $r'>j'$ then $\delta_{r'-1} + \delta_{r'-2} + \dots +\delta_{r} > \delta_{j'-1} + \delta_{j'-2} + \dots +\delta_{j}$, and viceversa if $r'<j'$.
    Hence, $\Delta_{j',j}\neq \Delta_{r',r}$.  
    
    The distance from any parent in set $S_{j}$ to any parent in  set $S_{j'}$ has the same integer part $\Delta_{j',j}$ and similarly the distances between parents in $S_r$ and in $S_{r'}$ have integer part $\Delta_{r',r}$, thus proving the claim. 
    
    We now consider the case of a pair of children $c < c'$
    \todoMR{}{$c$ potrebbe essere un filo problematico come nome}
    in different sets $j,j'$ (when they are in the same set their relative distance is the same of their parents).
    Let $p<p'$ be their respective parents. Hence, $\tau(c) = \tau(p) + \delta_j$ and $\tau(c') = \tau(p') + \delta_{j'}$. Therefore, $\tau(c') - \tau(c) =\tau(p') - \tau(p) + \delta_{j'} - \delta_j$.
    The integer part of $\tau(c') - \tau(c)$ is 
    \begin{equation}\label{eq-Gamma-ij}
        \Gamma_{j',j} = \Delta_{j',j} + \delta_{j'} - \delta_j = j'-j-1 + \delta_{j'} + \delta_{j'-1} + \dots +\delta_{j+1}.
    \end{equation}
    
    With the same reasoning used for the parents case, 
    $\Gamma_{j',j}\neq \Gamma_{r',r}$ if $r'\neq j'$: no two pairs of children may have the same integer distance, apart from those in the same set.  
    
    Let us now consider the case of a parent $p$ and a child $c'$ in different sets $j,j'$, with $c' > p$, hence $j' > j$.
    Let $p<p'$ be the parent of $c'$.
    Hence, $\tau(c') = \tau(p') + \delta_{j'}$. Therefore, $\tau(c') - \tau(p) =\tau(p') - \tau(p) + \delta_{j'}$.
    The integer part of $\tau(c') - \tau(p)$ is 
    \begin{equation}\label{eq-Theta-ij}
        \Theta_{j',j} = \Delta_{j',j} + \delta_{j'} = j'-j-1 + \delta_{j'} + \dots +\delta_{j}.
    \end{equation}
    
    Finally, we consider the case of a child $c$ and a parent $p'$ in different sets $j,j'$, with $p' > c$, hence $j' > j$.
    Let $p<p'$ be the parent of $c$.
    Hence, $\tau(c) = \tau(p) + \delta_{j}$. Therefore, $\tau(p') - \tau(c) =\tau(p') - (\tau(p) + \delta_{j})$.
    The integer part of $\tau(p') - \tau(c)$ is 
    \begin{equation}\label{eq-Xi-ij}
        \Xi_{j',j} = \Delta_{j',j} - \delta_{j} = j'-j-1 + \delta_{j'-1} + \dots +\delta_{j+1}.
    \end{equation}
    
    
    With the same reasoning used for the parents case, 
    $\Theta_{j',j}\neq \Theta_{r',r}$ if $r'\neq j'$: no two pairs parent-child children may have the same integer distance, apart from those in the same set.
    Similarly for $\Xi_{j',j}\neq \Xi_{r',r}$.
    
    Also, the expression of $\Gamma_{j',j}$ cannot be equal to any value $\Delta_{r',r}$, i.e., the integer distance of $c,c'$ is different from the distance of any pair of parents: 
    the first part of expression \eqref{eq-Gamma-ij}---i.e., the ``small'' integer
    component $j'-j-1$ (with $j'-j<n<\delta_1$)---can only appear in $\Delta_{j',j}$ but the second part---i.e., the ``large'' integer $\delta_{j'} + \delta_{j'-1} + \dots +\delta_{j+1}>2^j+2^{j+1}$---can only appear in 
    $\Delta_{j'+1,j+1}$. 
    Similarly for all pairs of $\Delta_{r',r}$, $\Gamma_{j',j}$, $\Theta_{b',b}$ and $\Xi_{o',o}$.
    \todoMR{}{Sistemato, ma si potrebbe ripulire}
    
    
    
    
    
    We now claim  that:
    
    \noindent (*) The distance between any two timestamps of positions in $S_1 \cup S_2 \dots \cup S_n$ is either less than 1 or greater than $\cmax$.  
    
    To prove the claim, define first the value $\alpha_j$ as  $\alpha_j = \tau(h+k-1)- \tau(h)$, when $h$ is the position of the leftmost parent in $S_j$ (and $h+k-1$ is the position of the rightmost). 
    Therefore, $\alpha_j = \tau(h+k-1)- \tau(h)= \frac{1}{2^{n+h}} (1-\frac{1}{2^{k-1}})< \frac{1}{2^{n}}$.
    
    It is then immediate to see that the timestamps of the parents in set $S_j$ are included in the  interval 
    \begin{equation}\label{eq-firstInterval}
        \left[d_{j}-\frac{j+1}{2^n}, d_{j}-\frac{j+1}{2^n}+\alpha_j\right].
    \end{equation}
    
    
    
    Thus  their children (at the fixed distance $\delta_j$) are in the interval (of length $\alpha_j$):
    
    \begin{equation}\label{eq-secondInterval}\left[d_{j}+\delta_j-\frac{j+1}{2^n}, d_{j}+\delta_j-\frac{j+1}{2^n}+\alpha_j\right]=\left[d_{j+1}-1-\frac{j+1}{2^n}, d_{j+1}-1-\frac{j+1}{2^n}+\alpha_j\right], 
    \end{equation} 
    
    
    
    Notice that, by~\eqref{eq-firstInterval}, if $j<n$, then the parents in set $S_{j+1}$ are in the interval (of length $\alpha_{j+1}$): 
    \begin{equation}\label{eq-nextInterval}\left[d_{j+1}-\frac{j+2}{2^n}, d_{j+1}-\frac{j+2}{2^n}+\alpha_{j+1}\right],
    \end{equation} 
    which is disjoint from the open interval~\eqref{eq-secondInterval} (because the left endpoint of \eqref{eq-nextInterval} is greater than the right endpoint of ~\eqref{eq-secondInterval}). 
    Therefore, the distance between any two points in the interval:
    
    $$\left[d_{j+1}-1-\frac{j+1}{2^n},d_{j+1}-\frac{j+2}{2^n}+\alpha_{j+1}\right],$$
    obtained by considering the left endpoint of \eqref{eq-secondInterval} and the right endpoint of  \eqref{eq-nextInterval}, is always less than 1, since the interval has length 
    $1+\frac{j+1}{2n}-\frac{j+2}{2^n}+\alpha_{j+1} = 1 -\frac{1}{2^n}+\alpha_{j+1}<1$, since $\alpha_{j+1}<\frac{1}{2^n}$.
    
    Therefore, in all the above cases the distance between any two timestamps in $(\pi,\tau)$ is less than 1 (e.g., the distance between the children in the $j$-th set and the parents in the $j+1$-th set), while in the remaining cases must it be greater than $\cmax$.  
    
    Thus, clocks can meaningfully be  compared only with parameters, since this is the only way to check for equality against values greater than $\cmax$ or less than 1.
    
    
    
    We  claim that for every $1\le j \le n$ there is at least one parameter, denoted as $\param_j$, which cannot be used for checking the transitions of children of any other set. Part (1) of the theorem then follows immediately, since we have $n+1$ sets and $n$ parameters. 
    \todoMR{}{questo deriva dalla riga 174, no?}
    
    In fact, by (*), a transition for a child in position, say, $h$, of  set $S_j$, $j>0$, can be enforced if, and only if, a clock can be compared for equality with a parameter. Such clock must have been reset in a previous position, say, $m<h$ hence the value of the parameter is $\tau(m)-\tau(h)$, which by \eqref{eq-allDistinct} is different from any other distance between a pair of positions, unless the position $m$ corresponds to the parent of position $h$: in the latter case, the distance is $\delta_j$, which is an integer unique to $S_j$. Therefore, the value of the parameter used in this comparison cannot be used for checking transitions of children of different sets. Thus, the claim is proved.
    
    
    We prove now part (2), where we consider the case of a TA where the number of clocks is $k$ or greater, but the number of parameters is less than $n$.  
    Recognizing the portion of the timed word over the language $(L^p_{k})^n$ requires at least $n$ parameters, for the reasons already explained. The above argument on this portion did not use any assumption on the number of clocks, so no parametric TA with less than $n$ parameters can recognize $(L^p_{k})^n$.
\end{proof}

By considering Lemma \ref{lm:LPk-not-k-1} with $n =1$ we immediately have the following corollary.

\begin{corollary}
    \label{thm:perTAmoreexpr}
    Parametric nrtTA are strictly more expressive than TA.
\end{corollary}





The following Theorem is an immediate consequence of Lemmata~\ref{lm:fromTAtonrtTA2} and \ref{lm:LPk-not-k-1}.



\begin{theorem}
    \label{thm:nrtTAngtTAltn}
    Parametric nrtTA with $k$ clocks and $n$ parameters (with $n, k \geq 1$) are strictly more expressive than parametric TA with $n$ parameters and less than $k$ clocks.
\end{theorem}



We also have the following result.

\begin{theorem}
    \label{thm:TAgtnrtTA}
    Parametric TA with $k$ clocks and $n$ parameters (with $n, k \geq 1$) are strictly more expressive than parametric nrtTA with $k$ clocks and $n$ parameters.
\end{theorem}

\begin{proof}
    Consider the language $\tilde{L}^{p}_k$, defined as the language $\bar{L}^{p}_k$ of Lemma~\ref{lm:LPk-not-k-1}, with the added constraint that $\tau(k) < 1$ (i.e., the first $k$ elements of the timed word all occur before one time instant). It is easy to see that $\tilde{L}^{p}_k$ can be recognized by a parametric TA with $k$ clocks and $n$ parameters.
    Assume by contradiction that there is a parametric nrtTA $\A$ recognizing $\tilde{L}^{p}_k$. Let $\cmax\ge 1$ be the largest constant in the guards of $\A$.
    
    
    Consider the timed word  $(\pi,\tau)$ defined in the proof of Lemma~\ref{lm:LPk-not-k-1}. 
    
    
    
    
    
    Consider now the first set $S_0$ of $k$-pairs, i.e, those in ${L}_k$ with $\tau(k)<1$.
    With the usual standard argument, any accepting run of $A$ over $(\pi,\tau)$ must be such that there is a transition precisely at each time instant $\tau(i+k) = \tau(i)+ 1$,
    $1\le i \le k$, hence at least one clock must reach either an integer value or some parameter
    value; but the latter case is impossible since, as already proved in  Lemma~\ref{lm:LPk-not-k-1}, at least $n$ parameters are needed to check the portion of the timed word in $({L}^{p}_k)^n$ and their values cannot be used to check the transitions of the portion in $L_k$. Since all clocks must have a value between 0 and 2 in the portion of the run in $L_k$, at every position $k+1, \dots, 2k$  one of the clocks must reach exactly the value 1 (hence it cannot reach any other integer in interval $(0,2)$).
    \todoMR{}{forse la parentesi è overkill}
    Since the distance between the element in a position $j$ and the one in position $j+k$ ($1\le j\le k)$ is exactly one, then a distinct clock is reset at each position $1, \dots, k$. 
    In position $k$, one clock is reset, say, $x$,  and the other clocks are greater than 0 and less than $1$. Since $\A$ is nrtTA, it cannot check the value of clock $x$, hence it cannot distinguish the case of this timed word from the case where we let $\tau(k)=1 +\varepsilon$, $\tau(2k)= 2+\varepsilon$, for some $\varepsilon>0$ such that $\varepsilon < \tau(1)$. Therefore, $\A$ may recognize timed words not in $\bar{L}^{p}_k$, a contradiction.
\end{proof}

